End-to-end people detection in crowded scenes

Current people detectors operate either by scanning an image in a sliding window fashion or by classifying a discrete set of proposals. We propose a model that is based on decoding an image into a set of people detections. Our system takes an image as input and directly outputs a set of distinct detection hypotheses. Because we generate predictions jointly, common post-processing steps such as non-maximum suppression are unnecessary. We use a recurrent LSTM layer for sequence generation and train our model end-to-end with a new loss function that operates on sets of detections. We demonstrate the effectiveness of our approach on the challenging task of detecting people in crowded scenes.

==> model.tex <==
\section{Loss Function - Discussion} 

We trained a network to output a list of bounding boxes for an image. There are a few natural choices for the loss function. One straight-forward option would be to arrange the ground truth boxes in some canonical ordering (e.g. left to right, top to bottom). Once ordered, train the LSTM to output the $i^{th}$ box's center, width, and height on the $i^{th}$ recurrent step. However, to see a limitation of this approach, consider what will happen if an image has three people arranged left to right, and the network fails to detect the middle person. At the first step of the LSTM, the network will output a box near the leftmost person, and perhaps receive some feedback on how to fine tune any minor errors in the exact center, width, and height of its prediction. On the second step, the network will erroneously skip the middle person and detect the rightmost. Intuitively, we would like to tell the network that it simply failed to detect the middle person. But instead, our loss function will tell the network that it's well localized detection should have output the center 100 pixels to the left. This is very strange feedback to give indeed! So, while the global minimum of this loss function may be a perfect set of bounding boxes, it fails to assign partial credit in a satisfactory manner.

In fact, any method that requires assigning a topological ordering to the ground truth boxes will be vulnerable to such gaps in the predicted ordering. What we really want is a loss function that doesn't worry too much about the order in which the boxes are output. Furthermore, we'd like to distinguish errors in detection from errors in localization, so that mistakes in the former don't dominate updates to the latter. To achieve these semantics, we developed a new loss function, which is one of the primary contributions of this paper. The high level idea is to generate an over-complete set of candidate boxes from the LSTM, in order of roughly descending confidence. False positive candidates are trained to have low confidence. True positive candidates are trained to have high confidence and correct localization. In what follows, we describe the details of the loss function. An application of our method to a new highly challenging data set and a discussion of the performance will follow thereafter.

\section{Architecture}

We use the bvlc-googlenet architecture provided by Caffe and pretrained on ImageNet. We discard the final fully connected layers, such that our input 480x640x3 image is transformed into a 15x20x1024 block of high level features.  we reshape these features into a 300x1024 block, with each 1024-d vector  describing the  bounding boxes surrounding each of the 300 cells in a 15x20 grid. Each 1024-d vector becomes the recurring input to an independent LSTM described below.





% We now define a loss functions used to train the network. The loss is defined on two sets of hypothesis. Set of candidate hypothesis generated by the model denoted as $C$ and set of ground-truth hypothesis $G$. 



% Hypothesis $\bvb^i \in C$ include box location and confidence. The loss function should encourage configurations of boxes that align well with $G$. That means close proximity in image space. The loss function should encourage confidence $b^i_c$ to be high on boxes close to ground-truth and low otherwise. In addition the loss function should penalize model outputs that generate multiple high-confident boxes for a single ground-truth hypothesis. Since we generate hypothesis sequentially we would also prefer the model to output correct hypothesis early on in the prediction process. 




% As a principled mechanism to enable loss function with above properties we propose a loss function based on finding optimal matching between elements of $C$ and $G$. 



% We use a simple example in Fig.~\ref{} to provide an illustration for the definition of the loss function. 







